Edge-as-a-Service: Towards Distributed Cloud Architectures

We present an Edge-as-a-Service (EaaS) platform for realising distributed cloud architectures and integrating the edge of the network in the computing ecosystem. The EaaS platform is underpinned by (i) a lightweight discovery protocol that identifies edge nodes and make them publicly accessible in a computing environment, and (ii) a scalable resource provisioning mechanism for offloading workloads from the cloud on to the edge for servicing multiple user requests. We validate the feasibility of EaaS on an online game use-case to highlight the improvement in the QoS of the application hosted on our cloud-edge platform. On this platform we demonstrate (i) low overheads of less than 6%, (ii) reduced data traffic to the cloud by up to 95% and (iii) minimised application latency between 40%-60%.

==> discovery.tex <==
The EaaS platform as shown in the edge node layer requires a master node (located in the edge node layer or elsewhere) and a collection of edge nodes. The master node executes an EaaS controller that connects to a collection of edge nodes. Each edge node executes an EaaS manager. The Master Node Controller comprises the following six modules (refer Figure~\ref{fig:figure2}).

\begin{figure}[t]
	\centering
	\includegraphics[width=0.6\textwidth]{images/figure2.png}
	\caption{Component view of the EaaS platform}
	\label{fig:figure2}
\end{figure}


1) The \textit{Master Node Manager} is the interface between the user input from the Web Application and the Master Controller. This module interacts with the Monitor and the Key Generator. User related information to isolate users is maintained by the User Database on the Master Node. The Edge Database contains information on all edge nodes that have been discovered and have installed an Edge Manager on the edge node.

2) The \textit{Monitor} periodically obtains key metrics, such as the CPU and memory utilisation from each edge node. The frequency of obtaining this information can be set by the Administrator. However, currently this module is centralised and we anticipate that it will be less scalable. Alternate distributed monitoring mechanisms will need to be implemented to make the EaaS platform more scalable.

3) The \textit{Key Generator} enhances security of the EaaS platform by generating a public and private key for containers. Users are provided can download a private key via the Web Application when a container is launched for the first time. 

4) The \textit{User Database} maintains the users of the EaaS system by managing usernames and passwords. The current active users on the edge nodes and their time of activity are logged in this database. 

5) The \textit{Edge Database} stores the information of all discovered edge node, such as its public IP, open port number and coordinator information and of containers on the edge node, such as its name, state and public IP.

\begin{table*}[ht]
\centering
\caption{Notation used in the proposed EaaS platform}
\begin{tabular}{c p{8cm} p{2cm}} \hline
\textbf{Parameter} & \textbf{Description} & \textbf{Source} \\ \hline
\(Prt_{controller}\) & Port used on controller for communication with edge nodes & \multirow{ 4}{*}{Master Node Controller}\\ 
\(IP_{controller}\) & IP address of the controller & \\ 
\(E\) & A set of $n$ edge nodes offered as a service, $e_i \in E, i=1,..., n$, where $e_i$ = [$IP_{e_i}$] & \\
\(C\) & A set of $m$ containers launched on $E$, $c_i \in C, i=1,..., m$, where $c_i$ = [$IP_{c_i}, status_{c_i}$] & \\
\hline
\(IP_{e_i}\) & IP address of edge node $e_i$ & \multirow{ 8}{*}{Edge Node}\\
\(Prt_e\) & Port used on edge nodes for communication with controller & \\
\(offer_i\) & A list of $[e_i,IP_{e_i},Prt_e]$ to offer services on edge node $e_i$ & \\
\(service\) & Flag on the availability of the services on an edge node & \\
\(key_{c_i}\) & Private key generated for accessing $c_i$ & \\
\(result_i\) & Results generated by an application in $c_i$ & \\
\(IP_{c_i}\) & IP address of container $c_i$ & \\
\(status_{c_i}\) & Status of container $c_i$ & \\
 \hline
\(conType\) & Flag for whether an Operating System (OS) or application container is deployed & \multirow{ 3}{*}{Edge Service User}\\
 \(action_i\) & Actions (launch, terminate, start or stop) on a container $c_i$  & \\
\(request_i\) & A list of $[conType, e_i, action_i, c_i]$ to request services on edge node $e_i$ & \\

\hline
\end{tabular}
\label{tab:table1}
\end{table*}

6) The \textit{Master Node Communicator} is the interface between the Controller and the Edge Node and communicates with edge node manager. Commands to launch, start, stop and terminate containers on the edge nodes are assembled in this module. The results of executing the commands on the edge node are obtained from the Edge Node Manager and used to update the database. Additionally, the metric information obtained from Monitoring is obtained by the Monitor via this module.

The \textit{Edge Node Manager} is installed on the edge node during discovery and executes commands obtained from Master Node Communicator and provides the output of the execution back to the Communicator. 

The \textit{Web Application} provides a user interface for accessing the EaaS platform. The users may be administrators of the EaaS platform or application owners who require access to an edge node. The administrator interface provides global information on a variety of metrics, such as CPU utilisation and memory utilisation of containers that are deployed by users on the edge node. The administrator can start, stop or terminate containers that are running. The application owner interface provides information relevant to the containers that a user has deployed on an edge node. The users can choose to launch an application container (for example, Docker) or an Operating System container (for example, LXD) on the edge node.

==> results.tex <==
The experiments we perform are firstly to demonstrate the low overhead of the discovery protocol. We observe that up to 50 containers were discovered on an edge nodes with less than a ten second overhead. These nodes are then made publicly and securely accessible for users by keys that are generated for individual users to access containers on the edge node. 
Then we demonstrate that the resource provisioning mechanism for offloaded workloads onto an edge node for servicing user requests improves QoS. We observe that data traffic to the cloud is reduced by up to 95\% when over 16,000 users are connected to a single edge node hosting 128 servers. The application latency is noted to reduce between 20\%-80\%.
Finally, we prove that dynamic auto-scaling reduces the Service Level Objective SLO violation rates for the use-case. In our set up SLO violations are reduced by up to 25\% when compared to not having auto-scaling. The merit of the mechanism is observed in that it has less than a 10 millisecond overhead when hosting 128 servers.  
